Classical (Co)Recursion: Mechanics

Primitive recursion is a mature, well-understood topic in the theory and practice of programming. Yet its dual, primitive corecursion, is underappreciated and still seen as exotic. We aim to put them both on equal footing by giving a foundation for primitive corecursion based on computation, giving a terminating calculus analogous to the original computational foundation of recursion. We show how the implementation details in an abstract machine strengthens their connection, syntactically deriving corecursion from recursion via logical duality. We also observe the impact of evaluation strategy on the computational complexity of primitive (co)recursive combinators: call-by-name allows for more efficient recursion, but call-by-value allows for more efficient corecursion.

==> sec_corec-fun.tex <==
\section{Recursion in the Lambda-Mu Calculus}
\label{sec:corec-fun}

We saw how co\-recursion, and not just co\-iteration, can be expressed inside
an abstract machine.  How can co\-recursion be seen in a more familiar language
similar to System T?

Our key insight is that the generality of co\-recursor is made possible by
\emph{control effects} equivalent to Scheme's \texttt{call/cc} operator.  The
co\-recursive branch is given access to two continuations: one to update the
accumulator and continue the co\-recursion, and the other to end co\-recursion
early by providing another stream in its entirety.

\begin{figure}
\begin{align*}
  A, B
  &::= A \to B \mid \Nat \mid \Stream A
  \\
  J, L
  &::= \cut{M}{Q}
  \\
  M, N
  &::= x
  \mid \outp\alpha J
  \mid \lambda x. M
  \mid M ~ N
  \\
  &\phantom{:=}
  \mid \Zero
  \mid \Succ M
  \mid \Rec M \As \ \{\Zero \to N \mid \Succ x \to y.M\}
  \\
  &\phantom{:=}
  \mid \Head M
  \mid \Tail M
  \mid \CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.M\}  \With M
  \\
  Q, R
  &::= \alpha
  \mid \inp x J
%  \\
%  \<ralt>
%  &::= \{\Zero \to N \mid \Succ x \to y.M\}
%  \\
%  \<calt>
%  &::= \{\Head \to x.N \mid \Tail \beta \to y.M\}
\end{align*}
\caption{Syntax of $\lambda\mu\tmu$ extended with (co)recursion.}
\label{fig:lambda-corec-syntax}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{1.0\linewidth}
\small
\begin{gather*}
  \infer[Cut]
  {\Gamma \entails \cut{M}{Q} \contra}
  {
    \Gamma \entails M \givestype A
    &
    \Gamma \entails Q \takestype A
  }
  \\[\ruleskip]
  \infer[Act]
  {\Gamma \entails \outp\alpha J \givestype A}
  {\Gamma, \alpha \takestype A \entails J \contra}
  \qquad
  \infer[CoAct]
  {\Gamma \entails \inp x J \takestype A}
  {\Gamma, x \givestype A \entails J \contra}
  \\[\ruleskip]
  \infer[{\Stream}I_{\Head}]
  {\Gamma \entails \Head M \givestype A}
  {\Gamma \entails M \givestype \Stream A}
  \quad
  \infer[{\Stream}I_{\Tail}]
  {\Gamma \entails \Tail M \givestype \Stream A}
  {\Gamma \entails M \givestype \Stream A}
  \\[\ruleskip]
  \infer[{\Stream}E]
  {
    \Gamma \entails
    \CoRec \{\Head \to x.N \mid \Tail \beta \to y.N'\} \With M
    \givestype \Stream A
  }
  {
    \Gamma, x \givestype B \entails N \givestype A
    &
    \Gamma, \beta \takestype \Stream A, y \givestype B \entails N' \givestype B
    &
    \Gamma \entails M \givestype B
  }
\end{gather*}
\end{minipage}
\caption{Type system for corecursion in $\lambda\mu\tmu$.}
\label{fig:lambda-corec-types}
\end{figure}

\begin{figure}
\small

Call-by-name values ($V$), co\-values ($K$), and evaluation contexts ($E$):
\begin{align*}
  V, W &::= M
  \qquad
  K, H
  ::= \alpha
  \\
  E,F
  &::= \hole
  \mid E ~ N
  \mid \Rec E \As \ \{\Zero \to N \mid \Succ x \to y.N'\}
  \mid \Head E
  \mid \Tail E
  \mid \cut{E}{K}
\end{align*}
Call-by-value values, co\-values, and evaluation contexts:
\begin{align*}
  V, W
  &::= x
  \mid \lambda x. M
  \mid \Zero
  \mid \Succ V
  \mid \CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.N'\}  \With V
  \\
  K, H &::= Q
  \\
  E,F
  &::= \hole
  \mid E ~ N
  \mid V ~ E
  \mid \Succ E
  \mid \Rec E \As \ \{\Zero \to N \mid \Succ x \to y.N'\}
  \\
  &\phantom{:=}
  \mid \Head E
  \mid \Tail E
  \mid \CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.N'\} \With E
  \mid \cut{E}{K}
\end{align*}
Operational reduction rules:
\begin{gather*}
\begin{aligned}
  (\mu)&&
  \cut{E[\outp\alpha J]}{K}
  &\srd
  J\subst{\cut{M}{\alpha}}{\cut{E[M]}{K}}
  \\
  (\tmu)&&
  \cut{V}{\inp x J} &\srd J\subst{x}{V}
  % \\
  % F[\outp\alpha J]
  % &\srd
  % \outp\beta J\subst{\cut{N}{\alpha}}{\cut{F[N]}{\beta}}
  \\
  (\beta_\to)&&
  (\lambda x. M) ~ V &\srd M\subst{x}{V}
  \\
  (\beta_{\Zero})&&
  \Rec \Zero \As \  \{\Zero \to N \mid \Succ x \to y.N'\}
  &\srd
  N
  \\
  (\beta_{\Succ})&&
  \Rec \Succ V \As \   \{\Zero \to N \mid \Succ x \to y.N'\}
  &\srd
  \outp\alpha\cut{\Rec V \As \  \{\Zero \to N \mid \Succ x \to y.N'\}
 }{\inp y \cut{N\subst{x}{V}}{\alpha}}
  % (\fn y N'\subst{x}{V}) ~ (\Rec V \As \<ralt>)
  % \Let y = \Rec V \As \<ralt> \In N'\subst{x}{V}
\end{aligned}
\\[1ex]
\begin{aligned}
  (\beta_{\Head})\quad&
  \Head (\CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.N'\} \With V)
  \srd
  N\subst{x}{V}
  \\
  (\beta_{\Tail})\quad&
  \cut{E[\Tail (\CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.N'\}  \With V)]}{K}
  \\
  &\srd
  \cut
  {
    E[
    \CoRec \  \{\Head \to x.N \mid \Tail \beta \to y.N'\}  \With
    N'\subs{\asub{y}{V},\asub{\cut{M}{\beta}}{\cut{E[M]}{K}}}
    ]
  }
  {K}
  % \\
  % &
  % \text{where } \rho = \subs{\asub{x}{V},\asub{\cut{M}{\beta}}{\cut{E[M]}{K}}}
\end{aligned}
\end{gather*}
%Where \begin{math}
%  \<ralt> \defeq \{\Zero \to N \mid \Succ x \to y.N'\}
%\end{math}
%and
%\begin{math}
%  \<calt> \defeq \{\Head \to x.N \mid \Tail \beta \to y.N'\}
%\end{math}
%above.
\caption{Operational semantics for (co)recursion in $\lambda\mu\tmu$.}
\label{fig:lambda-corec-operation}
\end{figure}

Our functional language for expressing co\-recursion is based on the
$\lambda\mu\tmu$-calculus \cite{DownenAriola2014CSCC}---an extension of
Parigot's $\lambda\mu$-calculus \cite{LambdaMu} with $\tmu$-abstractions---as
shown in \cref{fig:lambda-corec-syntax}.  In addition to everything from System
T, this language has $\mu$-abstractions ($\outp\alpha J$) and jumps ($\cut{M}Q$)
from the $\lambda\mu$-calculus, along with the dual $\tmu$-abstractions
($\inp x J$).  Intuitively, the $\mu\tmu$--abstractions serve the same role as
in the abstract machine---assigning a name to the continuation of a term or the
value given to a continuation, respectively---but now appear in the context of a
direct-style, functional language.

The co\-recursor $\CoRec \<calt> \With M$ appears almost the same as it
did in the abstract machine (albeit slightly generalized so that the accumulator
$M$ does not need to be a value), but the stream alternatives $\<calt>$ are
written in a different from, $\{\Head \to x.N \mid \Tail\beta \to y.M\}$, so
that co\-recursion can be written entirely with terms.  Similarly, the stream
projections now appear as terms rather than co\-terms.  $\Head M$ returns the
first element of a stream $M$, and $\Tail M$ returns the remaining elements of
$M$.  In total, the syntax of this $\lambda\mu\tmu$-calculus is biased toward
terms, where the only co\-terms are labels (\ie co\-variables $\alpha$) or
abstractions ($\inp x J$).

% The two dual abstractions $\outp\alpha J$ and $\inp x J$ allow us to express
% dual forms of $\Let$-bindings---one for binding the value of a term and one for
% binding the co\-value of a co\-term---as:
% \begin{gather*}
% \begin{aligned}
%   \Let x = M \In N
%   &\defeq
%   \outp\alpha \cut{M}{\inp x \cut{N}{\alpha}}
%   \\
%   \Let \alpha = Q \In R
%   &\defeq
%   \inp x \cut{\outp\alpha \cut{x}{R}}{Q}
% \end{aligned}
% \end{gather*}
% Note that this new macro-definition of $\Let$ is equivalent to the previous one
% in \cref{sec:rec-fun}, but it naturally exposes additional properties of $\Let$s
% that aren't immediately apparent in the encoding in terms of functions.%
% \footnote{For example, the $\beta_{\<lift>}$ \cite{ReasoningCPS}
%   axiom---$E[(\fn x M)~N] = (\fn x E[M])~N$---needed to complete the
%   call-by-value $\lambda$-calculus is directly derivable from the operational
%   semantics to follow.}
%
As before, we can macro-define the special cases for $\CoCase$ and $\CoIter$ as
ignoring the unneeded parameters of $\CoRec$ (and the unneeded accumulator for
$\CoCase$):
\begin{align*}
  \begin{alignedat}{2}
    \CoCase{}
    &\{
    \Head &&\to N
    \\
    &\mid \Tail &&\to M
    \}
  \end{alignedat}
  &\defeq
  \begin{aligned}
    &\CoRec
    \begin{alignedat}[t]{2}
      &\{~
      \Head &&\to \blank\,.N
      \\
      &\mid
      \Tail\alpha &&\to \blank\,. \outp\blank\cut{M}{\alpha}
      \}
      \\
      &\rlap{$\With \Zero$}
    \end{alignedat}
  \end{aligned}
  \\[0.5ex]
  \begin{aligned}
    &\CoIter
    \begin{alignedat}[t]{2}
      &\{~
      \Head &&\to x. N
      \\
      &\mid
      \Tail &&\to y.N'
      \}
      \\
      &\rlap{$\With M$}
    \end{alignedat}
  \end{aligned}
  &\defeq
  \begin{aligned}
    &\CoRec
    \begin{alignedat}[t]{2}
      &\{~
      \Head &&\to x. N
      \\
      &\mid
      \Tail\blank &&\to y.N'
      \}
      \\
      &\rlap{$\With M$}
    \end{alignedat}
  \end{aligned}
\end{align*}
The intuitive understanding is that $\CoCase$ introduces a stream whose first
element is exactly $N$ and remainder is $M$, analogous to $\<scons>$ previously
in \cref{sec:corec-mach}, so that:
\begin{align*}
  \Head(\CoCase \{\Head \to N \mid \Tail \to M\}) &= N
  \\
  \Tail(\CoCase \{\Head \to N \mid \Tail \to M\}) &= M
\end{align*}
As we saw with $\<scons>$, call-by-value evaluation reaches these results
directly but it may take (arbitrarily many) steps with call-by-name evaluation.
$\CoIter$ can be read as an endless loop that either returns the current element
(given by binding the value of $M$ to $x$ in $N$) or calculates the remaining
stream by updating its internal state (given by binding $M$ to $y$ in $N$).
However, there is no opportunity for $\CoIter$ to avoid updating the internal
state in the $\Tail$ case, and so the co\-iteration will continue no matter how
deeply the stream is inspected.

The type system for the (co)\-recursive $\lambda\mu\tmu$-calculus extends the
one for System T with additional typing rules given in
\cref{fig:lambda-corec-types}.  As with the abstract machine, we have judgments
for checking that a continuation $Q$ accepts an input of type $A$ (written
$\Gamma \entails Q \takestype A$) and that a jump $J$ is well-typed (written
$\Gamma \entails J \contra$).  Writing the type for a continuation of $A$ as the
negation $-A$ (recall \cref{rm:two-sided-sequent}), we can view the stream
operations as primitive constants with the following types:
%\begin{small}
\begin{align*}
  \Head &: \Stream A \to A
  \qquad
  \Tail : \Stream A \to \Stream A
  \\
  \CoCase_{\Stream A} &: A \to \Stream A \to \Stream A
  \\[0.25ex]
  \CoIter_{\Stream A}^B
  &:
  (B {\to} A) \to (B {\to} B) \to B \to \Stream A
  \\[0.25ex]
  \CoRec_{\Stream A}^B
  &:
  (B {\to} A) \to (-(\Stream A) {\to} B {\to} B) \to B \to \Stream A
\end{align*}
%\end{small}%

The operational semantics for (co)\-recursion is given in
\cref{fig:lambda-corec-operation}.  The rules for functions ($\beta_\to$) and
recursion ($\beta_{\Zero}, \beta_{\Succ}$) are the same as from
\cref{fig:t-operation}.  The $\mu$ rule states how the evaluation context is
captured by $\outp\alpha J$ and the $\tmu$ rule states how values are bound by
$\inp x J$, after which the jump $J$ is performed in either case.  The $\mu$
rule makes use of \emph{structural substitution} to substitute an evaluation
context ($E$) for a co\-variable ($\alpha$), written as
$J\subst{\cut{M}{\alpha}}{E[M]}$ in general, meaning that every jump of the form
$\cut{M}{\alpha}$ inside $J$ (where $\alpha$ appears free) is replaced by
$E[M]$.  Note that to be syntactically well-formed, the left- and
right-hand-sides of the $\mu$ rule are both jumps.\zena{TYPO, missing K. Needs jumps}
The $\beta_{\Head}$ rule
projects out the first element of a co\-recursive stream by substituting the
accumulator for the variable bound by the $\Head$ case.  The $\beta_{\Tail}$
rule projects out the remainder of a co\-recursive stream by updating the
accumulator.  This update performs two important bindings required by the
$\Tail$ case:
\begin{enumerate*}[(a)]
\item the current value of the accumulator is substituted for the bound
  variable, and
\item the current evaluation context is substituted for the co\-variable bound
  by the co\-pattern $\Tail\beta$.
\end{enumerate*}
As such, the $\beta_{\Tail}$ reduction may result in a new accumulator if this
computation returns normally, or it may jump to $\beta$ and provide an
altogether different stream.

The reduction theory of the (co)\-recursive $\lambda\mu\tmu$-calculus is written
as $J \to J'$ (and similar for (co)\-terms) and includes the compatible closure
of the operational rules (that is, they may be applied in \emph{any} context,
not just evaluation contexts).  We also include the following additional rule in
the reduction theory, which accounts for administrative reductions that bind
arbitrary terms inside of an evaluation context:
\begin{align*}
  (\varsigma)&&
  \cut{M}{\inp x E[x]}
  &\rd
  E[M]
\end{align*}
$\varsigma$ reduction completes the correspondence with the abstract machine,
given by this extension of the System T translation:
\begin{small}
\begin{align*}
\begin{aligned}
  \trans{\cut{M}{Q}} &\defeq \cut{\trans{M}}{\trans{Q}}
  \\[1ex]
  \trans{\alpha} &\defeq \alpha
  \\
  \trans{\inp x J} &\defeq \inp x \trans{J}
  \\[1ex]
  \trans{\Head M} &\defeq \outp\alpha \cut{\trans{M}}{\Head\alpha}
  \\
  \trans{\Tail M} &\defeq \outp\alpha \cut{\trans{M}}{\Tail\alpha}
  \\
  \trans{\CoRec \<calt> \With M}
  &\defeq
  \outp\alpha
  \cut{\trans{M}}{\inp x \cut{\CoRec \trans{\<calt>} \With x}{\alpha}}
\end{aligned}
\\[1ex]
\begin{aligned}
  &
  \trans{\{\Head \to x.N \mid \Tail\beta \to y.M\}}
  \\
  &\defeq
  \{
  \Head\alpha \to \inp x \cut{\trans{N}}{\alpha}
  \mid
  \Tail\beta \to \gamma. \inp y \cut{\trans{M}}{\gamma}
  \}
\end{aligned}
\end{align*}
\end{small}%
This translation preserves both the types and operations of the (co)\-recursive
$\lambda\mu\tmu$-calculus in the abstract machine (see \cref{sec:op-corr}).
\begin{restatable}[Type Preservation]{theorem}
  {thmcorectranstyped}
\label{thm:corec-trans-typed}
$\Gamma \entails J \contra$ in (co)\-recursive $\lambda\mu$ if and only if
$\Gamma \entails \trans{J} \contra$, and analogously for (co)\-terms.
\end{restatable}
\begin{restatable}[Operational correspondence]{theorem}
  {thmcorecopcorr}
\label{thm:corec-op-corr}
For any jump $\alpha\takestype\Nat\entails J \contra$ in (co)\-recursive
$\lambda\mu$, under both call-by-name and -value evaluation:
\begin{enumerate}
\item $J \srds \cut{\Zero}{\alpha}$ if and only if
  $\trans{J} \srds \cut{\Zero}{\alpha}$, and
\item $J \srds \cut{\Succ V}{\alpha}$ if and only if
  $\trans{J} \srds \cut{\Succ V'}{\alpha}$.
\end{enumerate}
\end{restatable}

The example streams $\<repeat>~x = x, x, x, \dots$ and
$\<alt> = 0, 1, 0, 1, \dots$ can be written in terms of co\-recursion like so:
%\begin{small}
\begin{align*}
  \<repeat>
  &\defeq
  \fn x
  \CoIter
  \{
  \Head \to y. y
  \mid
  \Tail \to z. z
  \}
  \With x
  \\
  \<flip>
  &\defeq
  \lambda x.
  \Case x \Of \{\Zero \to \Succ \Zero \mid \Succ \blank \to \Zero\}
  \\
  \<alt>
  &\defeq
  \CoIter
  \{
  \Head \to x.x
  \mid
  \Tail \to x.\<flip>~x
  \}
  \With \Zero
\end{align*}
%\end{small}%
Notice that the operational semantics of \cref{fig:lambda-corec-operation} gives
alternating outputs for the elements of $\<alt>$:
%\begin{small}
\begin{align*}
  \cut{\Head\<alt>}{\alpha}
  &\srd
  \cut{\Zero}{\alpha}
  \\
  \cut{\Head(\Tail\<alt>)}{\alpha}
  &\srds
  \cut{\Head\<alt'>}{\alpha}
  \srd
  \cut{\Succ\Zero}{\alpha}
  \\
  \cut{\Head(\Tail(\Tail\<alt>))}{\alpha}
  &\srds
  % \cut{\Head(\Tail\<alt>')}{\alpha}
  % \srds
  \cut{\Head\<alt>}{\alpha}
  \srd
  \cut{\Zero\!}{\alpha}
\end{align*}
%\end{small}%
and so on, where the intermediate state of the stream is
\begin{math}
  \<alt>'
  \defeq
  \CoIter
  \{
  \Head \to x.x
  \mid
  \Tail \to x.\<flip>~x
  \}
  \With \Succ\Zero
\end{math}.

\subsection{A corecursive coeliminator}
\label{sec:coelim}

Recall from \cref{sec:duality} that in the abstract machine, recursion and
co\-corecursion are perfectly dual to one another for dual types.  The recursor
has an internal state in the form of a co\-value (\ie continuation) keeping
track of the call stack built up by each step of recursion, whereas the
co\-recursor has an internal state in the form of a value (\ie accumulator)
that keeping of the progress made from one element to the next as projections
are made deeper into the stream.

Yet, in the $\lambda\mu\tmu$-calculus, the recursor and co\-recursor no longer
appear dual at all: the co\-recursor still has its internal state but the
recursor just returns a result, seemingly statelessly.  How can the duality
between these two forms be restored?  The mismatch is born from the fact that
introductions and eliminations of terms are \emph{not} dual to each other in the
sense we need.  Instead, an elimination of terms is symmetric to an
\emph{elimination of co\-terms}, \ie a \emph{co\-elimination}.
Co\-eliminators for functions have appeared before
\cite{StackCalculus,LambdaMuCons}, which has been used to study the issues of
confluence \cite{CBNExtConfluence} and head normalization
\cite{FirstClassCallStacks} with control effects.  We can derive a similar form
of co\-elimination for streams here, using $\tmu$-abstractions.  First, the
$\Head$ and $\Tail$ projections can be defined via macro-expansion as co\-terms
like so:
\begin{align*}
  \Head Q &\defeq \inp x \cut{\Head x}{Q}
  &
  \Tail Q &\defeq \inp x \cut{\Tail x}{Q}
\end{align*}
From there, we can give the following syntactic sugar for co\-recursion defined
by eliminating these two co\-terms:
\begin{gather*}
\begin{aligned}
  \begin{alignedat}{2}
    &\CoRec Q \As
    \\
    &\quad
    \{~
    \Head\alpha &&\to R
    \\
    &\quad
    \mid
    \Tail\beta &&\to \gamma.R'
    \}
  \end{alignedat}
  \defeq
  \begin{alignedat}{3}
    \inp x
    &\langle
    \CoRec{}
    &&\{~
    \Head &&\to z.\outp\alpha\cut{z}{R}
    \\
    &&&\mid
    \Tail\beta &&\to y.\outp\gamma\cut{y}{R'}
    \}
    \\
    &&&\With x
    \\[-1ex]
    &\cmid
    {~Q~}
    \rangle
  \end{alignedat}
\end{aligned}
\end{gather*}
The new definitions allow us to derive these reductions:
\begin{align*}
  \CoRec \Head K \As \<calt>
  &\rds
  R\subst{\alpha}{K}
  \\
  \CoRec \Tail K \As \<calt>
  &\rds
  \inp x \cut{\outp\gamma \cut{x}{R'\subst{\beta}{K}}}{\CoRec K \As \<calt>}
  % \Let \gamma = \CoRec K \As \<calt> \In R'\subst{\beta}{K}
\end{align*}
This provides us an alternative understanding of co\-recursion: rather than
focusing on generating some infinite object, we can instead focus on processing
a finite observation.  In other words, we can write co\-recursive definitions
in the same style as recursion on the natural numbers, with the twist that we
are calculating a question rather than an answer.

As an example, we can write definitions for the streams
\begin{small}
\begin{gather*}
  \<evens>~(x_0,x_1,\dots) = x_0,x_2,x_4,\dots
  \quad\!\!
  \<odds>~(x_0,x_1,\dots) = x_1,x_3,x_5,\dots
  \\
  \<merge>~(x_0,x_1,\dots)~(y_0,y_1,\dots)
  =
  x_0,y_0,x_1,y_1,\dots
\end{gather*}
\end{small}%
using pairs and the co\-eliminator above as follows:
\begin{small}
\begin{align*}
  \<evens>
  &\defeq
  \lambda s.\outp\gamma
  \langle
  {s}
  \cmid
  {
    \CoRec \gamma \As
    \begin{aligned}[t]
      \{&
      \Head \alpha \to \Head \alpha
      \\
      \mid&
      \Tail \blank \to \beta.\Tail(\Tail \beta)
      \}
      \rangle
    \end{aligned}
  }
  \\
  \<odds>
  &\defeq
  \lambda s.\outp\gamma
  \langle
  {s}
  \cmid
  {
    \CoRec \gamma \As
    \begin{aligned}[t]
      \{&
      \Head \alpha \to \Tail(\Head \alpha)
      \\
      \mid&
      \Tail \blank \to \beta.\Tail(\Tail \beta)
      \}
      \rangle
    \end{aligned}
  }
  \\
  \<merge>
  &\defeq
  \lambda s.\lambda s'\!.\outp\gamma
  \langle
  {(s,s')}
  \cmid
  {
    \CoRec \gamma
    \begin{aligned}[t]
      \{&
      \Head \alpha {\to} \inp{(s,\blank)}\cut{s}{\Head \alpha}
      \\
      \mid&
      \Tail \blank {\to} \gamma. \inp{(s,s')}\cut{(s'\!,\Tail s)}{\gamma}
      \}
      \rangle
    \end{aligned}
  }
\end{align*}
\end{small}%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "corec-prog"
%%% End:

